Event Generation with Sherpa 2.2

Sherpa is a general-purpose Monte Carlo event generator for the simulation of particle collisions in high-energy collider experiments. We summarize essential features and improvements of the Sherpa 2.2 release series, which is heavily used for event generation in the analysis and interpretation of LHC Run 1 and Run 2 data. We highlight a decade of developments towards ever higher precision in the simulation of particle-collision events.

==> macros.tex <==
\usepackage{amsmath}
\usepackage{amssymb}

\usepackage{axodraw}
\usepackage{wrapfig}
\usepackage{xspace}
\usepackage[usenames,dvipsnames]{xcolor}
\usepackage{graphicx}
\usepackage{setspace}
\usepackage{threeparttable}
\usepackage{relsize}
\usepackage{ifthen}
\usepackage{lineno}
\usepackage{enumerate}
\usepackage{makeidx}
\usepackage{showidx}

\setlength{\parindent}{0.0in}
\setlength{\parskip}{0.0in}

%%% Structuring
\newcommand{\Vp}{\ensuremath{\vphantom{\frac{|^|}{|^|}}}}
\newcommand{\LINE}{\underline{\hspace*{13.5cm}\hphantom{t}}\\}
\newcommand{\comment}[2][]{\noindent\LINE{\bf{#1}: }{#2}\\\LINE}
%\newcommand{\todo}[1]{\textbf{\color{red}#1}}
%\newcommand{\didit}[1]{\textbf{\color{blue}did it (#1)}}
%\newcommand{\checked}[1]{\hfill{\textbf{\color{green}\checkmark(#1)}}}
\newcommand{\todo}[1]{\fbox{\begin{minipage}{\textwidth}\textbf{#1}\end{minipage}}}
\newcommand{\didit}[1]{\textbf{\underline{#1}}}
\newcommand{\checked}[1]{\hfill{\textbf{\underline{#1}}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Maths macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{macros_maths}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Physics macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{macros_physics}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Section references
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{macros_refs}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Experiments / Machines
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{macros_collabs}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Software names
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{macros_codes}





==> text/amegic.tex <==
\subsection{\texorpdfstring{\protect\Amegic}{Amegic}}
\label{sec:me:amegic}

\Amegic \cite{Krauss:2001iv} is a tree-level matrix element generator
which, given some partonic process to be calculated, constructs the
full set of contributing tree-level Feynman diagrams which are in turn
translated into helicity amplitudes relying on a formalism similar to
the one described in \cite{Kleiss:1985yh,*Ballestrero:1992dv}. The
resulting expressions are written to \cpp code libraries which are
compiled and linked to \Sherpa in a semi-automatic fashion. The set of
Lorentz and colour structures supported by \Amegic allows for
calculations of in principle arbitrary scattering processes in the
standard model and simple extensions thereof, such as the effective
theory of gluon and photon interactions with the Higgs boson
\cite{Shifman:1979eb,Vainshtein:1980ea,Voloshin:1985tc}.

Dipole subtraction terms as used in the Catani--Seymour subtraction
scheme for NLO calculations are generated by \Amegic based on its
tree-level amplitudes as described in \cite{Gleisberg:2007md}.

For an efficient sampling of the phase space, \Amegic also generates
process specific phase space point generators. For each contributing
Feynman diagram, a generator channel is constructed based on the
diagram's resonance structure. Each channel is further dynamically
optimised by invoking the Vegas algorithm \cite{Lepage:1980dq}. All
channels are then combined into a variance-reducing self-adapting
multi-channel phase space generator based on the techniques outlined
in \cite{Kleiss:1994qy,Berends:1994pv,Ohl:1998jn}.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../sherpa"
%%% End:


==> text/summary.tex <==
\section{Summary}
\label{sec:summary}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../sherpa"
%%% End:

